Web-based Interactive Narratives to Present Business Processes Models

Interactive narratives offer a novel approach to presenting business process models, making them more accessible and collaborative. These narratives create a hyper-textual environment that facilitates knowledge exchange and comprehension for ordinary individuals. However, designing such narratives is complex, as business process modelers must accurately identify and translate the graphic elements of a process model into dynamic narrative elements. This research paper introduces the Scripting Your Process (SYP) method, which provides a systematic approach to designing interactive narratives based on business process models. Following the principles of Design Science Research (DSR), a quasi-experimental study demonstrates and evaluates the SYP method. The results show that the SYP method successfully achieves its objective, contributing to the systematic design of interactive narratives derived from business process models. Consequently, individuals who are not experts in business process management can understand these processes in an engaging and gameful manner.

==> Tables/questionario.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht!]
\centering
\caption{Perguntas do questionário de opinião}
\scriptsize
\label{tab:questionario}
%\begin{tabular}{|c|p{3.5cm}|c|}
\begin{tabular}{|c|p{8.5cm}|c|}


\hline
\textbf{Dimensão}                                                                                      & \textbf{Questão}                                                                                    & \textbf{Opções de Resposta}                                                                                        \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}(Q1)\\ Clareza e\\ Facilidade\end{tabular}}}        & Q1.1 - Qual o nível de dificuldade percebido na execução do método SYP?                                 & \begin{tabular}[c]{@{}c@{}}Múltipla escolha:\\ Fácil, Moderado ou Difícil\\ +\\ 2 Respostas Discursivas\end{tabular} \\ \cline{2-3} 
                                                                                                       & Q1.2 - O pré-roteiro gerado método SYP facilitaria o desenvolvimento da narrativa para o JDBPN?                      & \begin{tabular}[c]{@{}c@{}}Múltipla escolha:\\ Sim, Talvez ou Não\\ +\\ Resposta Discursiva\end{tabular}             \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}(Q2)\\ Viabilidade \\ de \\Uso\end{tabular}}}                     & Q2.1 - É possível gerar um pré-roteiro através do método SYP que represente o modelo de processo de negócio?              & \begin{tabular}[c]{@{}c@{}}Múltipla escolha:\\ Sim, Talvez ou Não\\ +\\ Resposta Discursiva\end{tabular}             \\ \cline{2-3} 
                                                                                                       & Q2.2 - Apenas com o modelo de processo de negócio é possível desenvolver o pré-roteiro de um JDBPN com o método SYP? & \begin{tabular}[c]{@{}c@{}}Múltipla escolha:\\ Sim, Talvez ou Não\\ +\\ Resposta Discursiva\end{tabular}             \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}(Q3)\\Utilidade\end{tabular}}                       & Q3.1 - Usaria o método SYP no caso de haver necessidade de desenvolver um JDBPN?                             & \begin{tabular}[c]{@{}c@{}}Múltipla escolha:\\ Sim, Talvez ou Não\\ +\\ Resposta Discursiva\end{tabular}             \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Opinião \\ Geral Sobre \\o  Método\end{tabular}}} & Aspectos positivos do método                                                                        & Resposta discursiva                                                                                                \\ \cline{2-3} 
                                                                                                       & Aspectos negativos do método                                                                        & Resposta discursiva                                                                                                \\ \cline{2-3} 
                                                                                                       & Sugestões de Melhoria                                                                               & Resposta discursiva                                                                                                \\ \hline
\end{tabular}
\end{table}

==> Tables/tbl_aswers_reviewers.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly

\footnotesize
\begin{longtable}[c]{|cp{5.0cm}p{5.0cm}c|}
\hline
\multicolumn{4}{|l|}{\textbf{Reviews "1" Comments}} \\ \hline
\endfirsthead
%
\endhead
%
\multicolumn{1}{|c|}{\textbf{Code}} &
  \multicolumn{1}{p{5.0cm}|}{\textbf{Comment}} &
  \multicolumn{1}{p{5.0cm}|}{\textbf{Answer}} &
  \textbf{Pages} \\ \hline
\multicolumn{1}{|c|}{01} &
  \multicolumn{1}{p{5.0cm}|}{The main strengths of this paper are that it addresses an interesting and timely question, understanding conceptual business process models and improving and enhancing their understanding is very important. The paper is generally well written and structured.} &
  \multicolumn{1}{p{5.0cm}|}{We appreciate your appointments. Thank you for that.} &
  - \\ \hline
\multicolumn{1}{|c|}{02} &
  \multicolumn{1}{p{5.0cm}|}{"in my opinion, the authors need to clearly explain their motivation to create interactive narratives from business process models"} &
  \multicolumn{1}{p{5.0cm}|}{We agree with your comment. In the article's new version, we clarify our motivation because interactive narratives (IN) are a dynamic and alternative business process model, different from the static and textual model. People can simulate the process using this IN and learn from its execution.} &
  1 and 2 \\ \hline
\multicolumn{1}{|c|}{03} &
  \multicolumn{1}{p{5.0cm}|}{The significance of the study in relation to related research should be stated, to me it was not clear enough why the solution approach the author propose is better than alternatives, how it is new and in which case it can be useful, what is the difference between  the authors' approach and generating textual process description from Business Process Model (from BPMN model), isn't it another form of automatic generation of text from process models by transforming process model elements (pools, lanes, activities, standard start and end events, message events, etc.) into sentences (Leopold et al., 2013)? If this is the case, then how can the authors claim that there are no approaches in the literature that have proposed creating interactive narratives (which is textual narratives in this case) from business  process models. I think the findings and contributions should be discussed more, and the difference from the previous study should  be clearly shown, also suggesting the citation of more relevant literature. Leopold, H., Mendling, J., \& Polyvyanyy, A. (2012). Generating natural language texts from business process models. In Advanced Information Systems Engineering: 24th International Conference, CAiSE 2012, Gdansk, Poland, June 25-29, 2012. Proceedings 24 (pp. 64-79). Springer Berlin Heidelberg.} &
  \multicolumn{1}{p{5.0cm}|}{In the new version of the article, we tried to explain our motivation and proposal better. First, our goal was not to say that interactive narratives are better than textual or BPMN. Our goal was to present interactive narratives as an alternative way to modeling business processes, providing a dynamic visualization. Thus, these alternative models can enable people to simulate the process execution. Second, we understand some research about generating natural language texts from business process models, not only from Leopold but from Santoro, Azevedo, Van Der Aa (with Leopold), and other researchers. Besides, they are newer than 2013, and we add them as references. However, we did not find research about "business processes" AND "interactive narratives" specifically. After searching in scientific bases such as Scopus, ACM, Science@Direct, and others, we did not find anything. We add this information in the section on related works. So, our research is different from others because of the interactive narratives used as alternative representations for business process models.} &
  1, 2, 4 and 5 \\ \hline
\multicolumn{1}{|c|}{04} &
  \multicolumn{1}{p{5.0cm}|}{The authors proposed to extract elements of a business process model to develop an interactive  narrative. What about the complex business process models? The authors did not specify the level of  complexity of these Business Process models; in some cases, BP models contain complex graphical  information that requires users to infer hidden behavior among process elements. In these cases, how  can the accuracy of the interactive narratives extracted from these elements be verified? In my  opinion, the authors should first evaluate the usefulness of interactive narratives and show the need  to design web-based interactive narratives from elements of business process models, then focus on  how to design them and finally evaluate the accuracy (semantically not only grammatically) of the  generated interactive narratives.} &
  \multicolumn{1}{p{5.0cm}|}{The complexity of the business process models is a limitation of this research, and we will work on it in the future. In this paper, we presented a method to support the design of interactive narratives using BPMN models relatively simple. That is, models that contain lanes, pools, simple tasks, events, etc. We add information about the BPMN complexity in the article. We said that even though the model was simple, it had all of the principal atomic elements used by process modelers to represent an organizational process. We understand that there are complex elements, such as subprocesses and bigger models. However, they will be targeted in future investigations and to improve the SYP method. We agree with your observation and will add this argumentation in the limitation section as a limitation in future works. Lastly, this research did not compare interactive narratives with BPMN or another visual model. Here, we evaluate if the SYP method could support process modelers to create interactive narratives in a complete correct, in systematic way. We will perform a model comparison in future work.} &
  17 and 18 \\ \hline
\multicolumn{1}{|c|}{05} &
  \multicolumn{1}{p{5.0cm}|}{Abstract accurately reflect the content of the article} &
  \multicolumn{1}{p{5.0cm}|}{We appreciate your appointments. Thank you for that.} &
  - \\ \hline
\multicolumn{1}{|c|}{06} &
  \multicolumn{1}{p{5.0cm}|}{The introduction did not provide enough background information for readers not in the immediate field to understand the problem and there is a lack of references to more recent literature. To make the introduction more substantial, I suggest rewriting the introduction. It needs to be more detailed. The authors need to present a background theory on interactive narratives and explain what the interactive narrative approach to business process is, why it is important and how it can affect the understanding of business process models.} &
  \multicolumn{1}{p{5.0cm}|}{In the new version, we rewrote the introduction and tried to improve our motivations and arguments. Also, we added more actual references.} &
  1 and 2 \\ \hline
\multicolumn{1}{|c|}{07} &
  \multicolumn{1}{p{5.0cm}|}{P1, §3, this is a very vague statement. The authors claims that interactive narratives can contribute to the understanding of business processes. on what basis has the author based his claims? the authors need to explain how.} &
  \multicolumn{1}{p{5.0cm}|}{We agree with you and rewrote the introduction to explain some affirmations better.} &
  1 and 2 \\ \hline
\multicolumn{1}{|c|}{08} &
  \multicolumn{1}{p{5.0cm}|}{The authors claim that no approach in related work has proposed the creation of interactive narratives from business process models. Although the related work referenced in this manuscript is dated, the paper lacks introducing more recent references. Did the authors provide a literature review analysis? If so, it is not mentioned anywhere within the manuscript.} &
  \multicolumn{1}{p{5.0cm}|}{We agree. We found more recent references and used them to support our argument. About the formal literature review, we answered in comment \#03.} &
  1, 2 and 4 \\ \hline
\multicolumn{1}{|c|}{09} &
  \multicolumn{1}{p{5.0cm}|}{The methodology section needs to be improved. Write clearly how the experiment was set up and conducted (clearly explain the data in Table 4). The method used should be justified by the authors} &
  \multicolumn{1}{p{5.0cm}|}{In the new version of the paper, we describe the quasi-experiment better.} &
  11 to 15 \\ \hline
\multicolumn{1}{|c|}{10} &
  \multicolumn{1}{p{5.0cm}|}{Fonts are too small to read in Figures 1, 3 and 4.  The figure (Fig. 2) does not display the order of execution of the two steps (sentence extraction and sentences scripting), the figure (Fig. 2) should be more explicit for the reader. The quality of figures (Figures 1,2, 3, 4) are not adequate for publication. I suggest to authors to use vector scale format (SVG). Figures and tables are not presented uniformly (for example, in the same format and fonts).} &
  \multicolumn{1}{p{5.0cm}|}{We adjusted tables and Figures. However, it is not possible to generate all of them as SVG because there are some print screens.  For Fig.1, we remake the figure and generate it in SVG. It is also valid for Fig 2 that we remake and add information on the execution of the SYP method.  Regarding the Fig. 3. We separated it into two figures and improved the resolution. We cannot generate SVG or change font style and size for Fig. 3, 4, 5, and 6 (new names) because they are printed from systems.  Tables use the font of the journal's template (Times New Roman), even though we uniformized their size.} &
  - \\ \hline
\multicolumn{1}{|c|}{11} &
  \multicolumn{1}{p{5.0cm}|}{The authors have validated its proposal through a quasi-experiment approach to analyze whether the SYP method is simple and useful for screenwriters in narrative design. The authors used a quasi-experimental empirical evaluation, which has less internal validity than true experiments - without randomization of the selection of the participants, it can be difficult to verify that all confounding variables have been taken into account. Furthermore, the number of participants is too small (only 19 participants), which may have an impact on the evaluation findings;} &
  \multicolumn{1}{p{5.0cm}|}{We agree that the number of participants is small. However, in an initial evaluation, the answers brought us insights and evidence to improve our research, and our approach seems valid. Nevertheless, we will put it in the limitation section, highlighting that it is necessary to perform new assessments with more people.} &
  17 \\ \hline
\multicolumn{1}{|c|}{12} &
  \multicolumn{1}{p{5.0cm}|}{The authors conducted an empirical evaluation in a quasiexperimental study with scriptwriters to analyze whether or not the method supports scriptwriters in creating correct interactive narratives according to a business process model. However, the authors did not show how to assess the semantic correctness of the generated interactive narratives.} &
  \multicolumn{1}{p{5.0cm}|}{We did not perform any semantic evaluation of the narrative interactive. We evaluate whether the amount of BPMN elements was present in the narrative and if they follow the process sequence correctly. We believe it could be a future evaluation that we can do. We will add it as future work in the limitation section. We thank you for mentioning that.} &
  17 \\ \hline
\multicolumn{1}{|c|}{13} &
  \multicolumn{1}{p{5.0cm}|}{No true experiments validation provided by the authors to verify the quality and the correctness of the provided scripts.} &
  \multicolumn{1}{p{5.0cm}|}{Sorry, but we did not do that. We think it could be a future step, but,  for this article, it is impracticable to execute it in time.} &
  - \\ \hline
\multicolumn{1}{|c|}{14} &
  \multicolumn{1}{p{5.0cm}|}{The literature cited is relevant to the topic, however, the related work referenced in this manuscript is dated, the paper lacks the introduction of more recent references.} &
  \multicolumn{1}{p{5.0cm}|}{Aswered in comment \#03.} &
  - \\ \hline
\multicolumn{1}{|c|}{15} &
  \multicolumn{1}{p{5.0cm}|}{There are several instances where the authors make assertions without substantiating them with references, for e.g. P1, §3.} &
  \multicolumn{1}{p{5.0cm}|}{We reformulated our sentences and tried to add references in our assertions, except when discussing interactive narrative as an alternative business process model because it is our proposal.} &
  1 and 2 \\ \hline
\multicolumn{1}{|c|}{16} &
  \multicolumn{1}{p{5.0cm}|}{Conclusion section can be enhanced. It would also be interesting to look at the impact of its work from a Business expert perspectives.} &
  \multicolumn{1}{p{5.0cm}|}{We agreed with the reviewer, and we improved the conclusions. We add many suggestions (evaluations with business experts, for instance) as limitations and for future works because it is impracticable to execute our experiment again with the time that we have. Also, this paper cannot analyze the research from a business expert's view. However, we consider it as a future analysis as an improvement of our proposal.} &
  18 \\ \hline
\multicolumn{4}{|l|}{\textbf{Reviews "2" Comments}} \\ \hline
\multicolumn{1}{|c|}{17} &
  \multicolumn{1}{p{5.0cm}|}{On page 2 in "The BPMN Language" there is a number that suggests a footer but it was not found} &
  \multicolumn{1}{p{5.0cm}|}{It was a little typing mistake. We apologize for this. We already corrected it in the new version of the article.} &
  2 \\ \hline
\multicolumn{1}{|c|}{18} &
  \multicolumn{1}{p{5.0cm}|}{Two references with the same authors and date must have a difference when mentioned (Gonçalves, Santoro \& Baião 2010, Gonçalves, Santoro \& Baiao 2010)} &
  \multicolumn{1}{p{5.0cm}|}{We appreciate the note. We had not realized that the Latex template would not put a letter after the year to differentiate the references. We put 2010a and 2010b to differentiate them.} &
  4 \\ \hline
\multicolumn{1}{|c|}{19} &
  \multicolumn{1}{p{5.0cm}|}{Write in more detail the profile of the participants in the experiment.} &
  \multicolumn{1}{p{5.0cm}|}{We agree with you and put more information about our participants' profiles.} &
  11 \\ \hline
\end{longtable}

\normalsize
\setcounter{table}{0}
\

==> Tables/tbl_inferential_estatistics.tex <==
\begin{table}[ht!]
\centering
\caption{Inferential statistics for Q1 and Q2}
\label{tab:inferential}
\footnotesize
\begin{tabular}{l|c|c|c|}
\cline{2-4}
 &
  \textbf{\begin{tabular}[c]{@{}c@{}}Normality Test\\ (Shapiro-Wilk)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Hypothesis Inference Test\\ (Wilcoxon)\end{tabular}} &
  \textbf{Result} \\ \hline
\multicolumn{1}{|l|}{\textbf{Q1}} &
  3.97E-08 &
  5.30E-05 &
  Alternative Hypothesis Accepted \\ \hline
\multicolumn{1}{|l|}{\textbf{Q2}} &
  1.18E-06 &
  7.76E-05 &
  Alternative Hypothesis Accepted \\ \hline
\end{tabular}
\end{table}

==> Tables/tbl_narrativa_bpmn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\caption{Mapeamento entre elementos narrativos e elementos BPMN}
\label{tab:narrativa_bpmn}
\scriptsize
\begin{tabular}{|p{1.8cm}|p{1.5cm}|p{2.0cm}|p{8.0cm}|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Elementos da Narrativa}}} & \multirow{2}{*}{\textbf{Elementos BPMN}}  & \textbf{Correspondência entre o Elemento da Narrativa e o Modelo do Processo}\\
\multicolumn{2}{|c|}{}                                        &                                  &                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{2}{|c|}{\textbf{Conflito}}                                & \textbf{Eventos, atividades e gateways}   & O conflito corresponde a uma instância do processo, com isso envolve um fluxo particular de eventos, atividades e gateways de acordo com as escolhas do jogador ao longo da trajetória da narrativa. Devem ser previstas as cenas para todos os conflitos possíveis.                                                                                \\ \hline
\multicolumn{2}{|c|}{\textbf{Personagens}}                                  & \textbf{Raias}                            & As raias representam atores do processo ou stakeholders e são os indicados para personagens história.     \\ \hline
\multirow{3}{*}{\textbf{Ação dramática}}         & \textbf{Primeiro ato (Início)}        & \textbf{Evento inicial, atividades}       & As cenas do primeiro ato, onde é introduzida a história e apresentado o conflito, estão associadas com o evento inicial do processo, mas também pode incorporar algumas atividades iniciais do fluxo.                                                                                                                                                                \\ \cline{2-4} 
                                        & \textbf{Segundo ato (Meio)}         & \textbf{Atividades, eventos intermediários e gateways}   & As cenas do segundo ato, onde o jogador supera os desafios e passa pelas provas para atingir o seu objetivo no jogo, estão associadas com as atividades que são desenvolvidas pelo ator correspondente no processo, com os eventos intermediários do processo e com as escolhas que são tomadas nesta trajetória, ou seja, as seleções de fluxo nos gateways. \\ \cline{2-4} 
                                        & \textbf{Terceiro ato (Conclusão)}        & \textbf{Evento final, atividades}         & As cenas do terceiro ato, onde acontece o desfecho da narrativa, estão associadas com o evento final do processo, além de eventualmente algumas atividades associadas com a finalização do processo (entrega de produto, por exemplo).                                                                                                              \\ \hline

\multicolumn{2}{|c|}{\textbf{Espaço}}                                  & \textbf{Raias}                            & O ambiente em que as cenas ocorrem correspondem a uma das raias do processo que indique o local, caso tenha sido mapeado no modelo.                                                                                                                                                                                                                 \\ \hline
\multicolumn{2}{|c|}{\textbf{Objetos}}                                 & \textbf{Artefatos (Recursos, Dados, etc.)} & Os objetos utilizados pelo jogador ao longo da cena estão associados com os artefatos do modelo do processo.                                                                                                                                                                                                                                          \\ \hline
\end{tabular}
\end{table}

==> Tables/tbl_narrativa_bpmn_copia.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\caption{Mapeamento entre elementos narrativos e elementos BPMN}
\label{tab:narrativa_bpmn}
\scriptsize
\begin{tabular}{|p{1.8cm}|l|p{2.2cm}|p{8.0cm}|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{\textbf{Elementos da Narrativa}}} & \multirow{2}{*}{\textbf{Elementos BPMN}}  & \textbf{Correspondência entre o Elemento da Narrativa e o Modelo do Processo}                                                                                                                                                  \\
\multicolumn{2}{|l|}{}                                        &                                  &                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{2}{|l|}{\textbf{Narrador}}                                & \textbf{Raias}                            & O narrador virá de uma das raias (lanes) do modelo BPMN, caso seja um narrador participante ou onisciente. Se for um narrador ausente, neste caso não há razão para identificar no modelo do processo.                                                                                      \\ \hline
\multicolumn{2}{|l|}{\textbf{Conflito}}                                & \textbf{Eventos, atividades e gateways}   & O conflito corresponde a uma instância do processo, com isso envolve um fluxo particular de eventos, atividades e gateways de acordo com as escolhas do jogador ao longo da trajetória da narrativa. Devem ser previstas as cenas para todos os conflitos possíveis.                                                                                \\ \hline
\multirow{3}{*}{\textbf{Personagens}}            & \textbf{Herói}               & \textbf{Raias}                            & Uma das raias que represente um papel relevante do processo é candidata a representar o herói da narrativa, podendo ser escolhida aquela que contenha as atividades que se queira retratar na narrativa, ou mais de um, caso o personagem mude de papel no decorrer da história.                                                                    \\ \cline{2-4} 
                                        & \textbf{Mentor}              & \textbf{Raias}                            & O mentor, caso exista, pode representar uma das raias que contenha um papel no processo, seja de liderança, supervisão ou mesmo de clientes, considerando que tenham um papel de guiar o herói em sua jornada.                                                                                                                                      \\ \cline{2-4} 
                                        & \textbf{Coadjuvantes}        & \textbf{Raias}                            & As raias que representem outros atores do processo (que não o herói ou o mentor) ou stakeholders são os indicados para personagens coadjuvantes na história.                                                                                                                                                                                        \\ \hline
\multirow{3}{*}{\textbf{Ação dramática}}         & \textbf{Primeiro ato}        & \textbf{Evento inicial, atividades}       & As cenas do primeiro ato, onde ocorre o chamado para a aventura, estão associadas com o evento inicial do processo, mas também pode incorporar algumas atividades iniciais do fluxo.                                                                                                                                                                \\ \cline{2-4} 
                                        & \textbf{Segundo ato}         & \textbf{Atividades, eventos intermediários e gateways}   & As cenas do segundo ato, onde o herói supera os desafios e passa pelas provas para atingir o seu objetivo, estão associadas com as atividades que são desenvolvidos pelo ator correspondente no processo, com os eventos intermediários do processo e com as escolhas que são tomadas nesta trajetória, ou seja, as seleções de fluxo nos gateways. \\ \cline{2-4} 
                                        & \textbf{Terceiro ato}        & \textbf{Evento final, atividades}         & As cenas do terceiro ato, onde acontece o desfecho da narrativa, estão associadas com o evento final do processo, além de eventualmente algumas atividades associadas com a finalização do processo (entrega de produto, por exemplo).                                                                                                              \\ \hline
\multicolumn{2}{|l|}{\textbf{Tempo}}                                   & \textbf{Eventos}                          & Caso o processo tenha "tempos" definidos na execução de seu fluxo, entre uma atividade e outra deve ter eventos de tempo para indicar isso, o que pode ajudar na definição do tempo para as cenas.                                                                                                                                                  \\ \hline
\multicolumn{2}{|l|}{\textbf{Espaço}}                                  & \textbf{Raias}                            & O ambiente em que as cenas ocorrem correspondem a uma das raias do processo que indique o local, caso tenha sido mapeado no modelo.                                                                                                                                                                                                                 \\ \hline
\multicolumn{2}{|l|}{\textbf{Objetos}}                                 & \textbf{Artefatos (Recursos, Dados etc.)} & Os objetos utilizados pelo herói ao longo da cena estão associados com os artefatos do modelo do processo.                                                                                                                                                                                                                                          \\ \hline
\end{tabular}
\end{table}
